Learned Semantic Multi-Sensor Depth Map Fusion

Volumetric depth map fusion based on truncated signed distance functions has become a standard method and is used in many 3D reconstruction pipelines. In this paper, we are generalizing this classic method in multiple ways: 1) Semantics: Semantic information enriches the scene representation and is incorporated into the fusion process. 2) Multi-Sensor: Depth information can originate from different sensors or algorithms with very different noise and outlier statistics which are considered during data fusion. 3) Scene denoising and completion: Sensors can fail to recover depth for certain materials and light conditions, or data is missing due to occlusions. Our method denoises the geometry, closes holes and computes a watertight surface for every semantic class. 4) Learning: We propose a neural network reconstruction method that unifies all these properties within a single powerful framework. Our method learns sensor or algorithm properties jointly with semantic depth fusion and scene completion and can also be used as an expert system, e.g. to unify the strengths of various photometric stereo algorithms. Our approach is the first to unify all these properties. Experimental evaluations on both synthetic and real data sets demonstrate clear improvements.

==> figs/eth3d_table.tex <==
\begin{table} 
\centering
\begin{tabular}{|c||c|c||c|c|}
\hline
Fusion & SA train & FA train & SA val & FA val \\
\hline
\hline
Average &  0.64 &  0.95   &  0.5  &  0.96  \\
\hline
Learned &  0.69  &  0.96  &  0.59 &  0.97   \\
\hline
\end{tabular}
\caption{ETH3D low res and high res. Semantic accuracy (SA) and free-space accuracy (FA). }\label{tab:eth3d}
\end{table}


==> figs/expert_table.tex <==
\begin{table} 
\centering
\begin{tabular}{c|c}
\hline
Used fusion & SA \\
\hline
\hline
Block Matching (BM)~\cite{sgbm} &   0.71  \\ 					      
% \hline
Semi-Global Block Matching (SGBM)~\cite{sgbm} &   0.71  \\ 	                                                  
% \hline
PSMNet~\cite{psmnet}  &  0.69   \\ 							      
% \hline
FCRN monocular~\cite{fcrn}    &   0.44  \\ 	         
% \hline
3 fusion (depth, grad mean) &    0.72 \\ 	                         
% \hline
3 fusion (depth, grad mean and std) &   0.725  \\ 	
% \hline
3 fusion (depth, grad mean and std, NCC)   &   0.735  \\ 	 
% \hline
4 fusion (depth, grad mean and std)      &   0.73  \\ 	                     
\hline
\end{tabular}
\caption{Expert system evaluation with 4 stereo methods: Block Matching (BM), Semi-Global Block Matching (SGBM), Pyramid Stereo Matching Network (PSMNet), Deeper Depth Prediction with Fully Convolutional Residual Networks (FCRN). The fusion are marked as follows: 3 fusion~--~SGBM+BM+PSMNet, 4 fusion~--~SGBM+BM+PSMNet+FRCN. Words in brackets denote the used input for confidence estimation: depth~--~average 3$\times$3 depth patches, grad mean~--~ mean gradient, grad std~--~standard deviation of gradient, NCC~--~average normalized cross correlation of 5$\times$5 patches of stereo images.}\label{tab:expert}
\end{table}


==> figs/scannet_table.tex <==
\begin{table} 
\centering
\begin{tabular}{|c|c|c|}
\hline
Fusion &  SA val & FA val \\
\hline
\hline
Average &  0.79 &  0.96   \\
% \hline
% Weighted Average &  0.83 &  0.97   \\
\hline
Learned &  0.9  &  0.97   \\
\hline
\end{tabular}
\caption{ScanNet evaluation. Semantic accuracy (SA) and free-space accuracy (FA). }\label{tab:scannet}
\end{table}


==> figs/suncg_table.tex <==
\begin{table} 
\begin{center}
\begin{tabular}{c|l}
\hline
Used fusion & SA \\
\hline
\hline
Stereo half 	&   0.68  \\ 					      
% \hline
Stereo full &   0.71  \\ 	                                                  
% \hline
Kinect half  &  0.73   \\ 							      
% \hline
Stereo half + Kinect half     &   0.76  \\ 	         
% \hline
Kinect full	                         &    0.77 \\ 	                         
% \hline
Stereo half + Kinect half (depth) &   0.77  \\ 	
% \hline
Stereo half + Kinect half (depth, gradient) &   0.78  \\ 	 
% \hline
Stereo full + Kinect full (depth, gradient) &   0.786  \\ 	                     
% \hline
Perfect sensor full  &   0.794  \\ 	
\hline
\end{tabular}
\end{center}
\caption{Ablation study on SUNCG. For each fusion approach we report semantic accuracy (SA). Depth means that average 3$\times$3 depth patch was included in the confidence estimation. Gradient denotes additionally mean and standard deviation of graient magnitudes. In case of \textit{half}, only half of the input images were used, whereas \textit{full} stands from the whole dataset. }\label{tab:suncg}
\end{table}

